Counterfactual Identifiability of Bijective Causal Models

We study counterfactual identifiability in causal models with bijective generation mechanisms (BGM), a class that generalizes several widely-used causal models in the literature. We establish their counterfactual identifiability for three common causal structures with unobserved confounding, and propose a practical learning method that casts learning a BGM as structured generative modeling. Learned BGMs enable efficient counterfactual estimation and can be obtained using a variety of deep conditional generative models. We evaluate our techniques in a visual task and demonstrate its application in a real-world video streaming simulation task.

==> sections/abstract.tex <==
\begin{abstract}
We study counterfactual identifiability in causal models with bijective generation mechanisms (BGM), a class that generalizes several widely-used causal models in the literature. We establish their counterfactual identifiability for three common causal structures with unobserved confounding, and propose a practical learning method that casts learning a BGM as structured generative modeling. Learned BGMs enable efficient counterfactual estimation and can be obtained using a variety of deep conditional generative models. We evaluate our techniques in a visual task and demonstrate its application in a real-world video streaming simulation task.
\end{abstract}

==> sections/ack.tex <==
\section*{Acknowledgements}
\label{sec:ack}

We would like to thank Behrooz Tahmasebi for discussions that led to the proof of \Cref{thm:IV}.
This work was supported by NSF grant 1751009, a gift from the CSAIL SystemsThatLearn (STL) Initiative, and Google, Intel, and Amazon as part of the MIT Data Systems and AI (DSAIL) lab.

==> sections/background.tex <==
\section{Preliminaries}
\label{sec:prelim}

We provide a brief background on the (mostly) causal concepts that we use in this work.
Refer to \citet{pearl2009causality}, \citet{pearl2009primer}, and \citet{peters2017elements} for more details.

\textbf{Notation:}
We refer to a random variable with a capital letter, e.g., $X$, the value it obtains with a lowercase letter, e.g., $x$, its Probability Density Function (PDF) with $P_X$, and a set of random variables with boldface font, e.g., $\boldsymbol{X} = \{X_1, \ldots, X_n\}$.
$J_{f(\cdot)}$ denotes the Jacobian of $f(\cdot)$.

\textbf{SCM and Causal Diagram:}
We use the framework of Structural Causal Models (SCMs)~\citep[Ch.~7]{pearl2009causality}.
An SCM $\mathcal{M}$ consists of endogenous variables $\boldsymbol{V}$ determined by other variables in the model, exogenous (also called latent or background) variables $\boldsymbol{U}$ with distribution $P_{\boldsymbol{U}}(\cdot)$ determined by factors outside the model (one exogenous variable corresponding to each endogenous variable), and generation mechanisms $\mathcal{F}$.
$\mathcal{F}$ contains a function $f_i$ for each variable $V_i$ that maps endogenous parents $\text{Pa}(V_i)$ and exogenous variable $U_i$ to $V_i$.
The entire $\mathcal{F}$ defines a structured mapping from $\boldsymbol{U}$ to $\boldsymbol{V}$.
The prior distribution over exogenous variables, $P_{\boldsymbol{U}}(\cdot)$, together with the generation mechanisms $(\mathcal{F})$ entail an observational $(\mathcal{L}_1)$ distribution over endogenous variables which we refer to as $P_{\boldsymbol{V}}^\mathcal{M}(\cdot)$.
Each $\mathcal{M}$ induces a causal diagram $\mathcal{G}$, where every $V_i \in \boldsymbol{V}$ is a vertex, there is a directed arrow $(V_j \rightarrow V_i)$ for every $V_i \in \boldsymbol{V}$ and $V_j \in \text{Pa}(V_i)$, and there is a dashed-bidirected arrow $(V_j \dashleftarrow \dashrightarrow V_i)$ for every $V_i, V_j \in \boldsymbol{V}$ such that $U_i$ and $U_j$ are not independent.
The bidirected arrows represent existence of unobserved confounders.
A causal model satisfies the \emph{Markovian} assumption if for every $V_i, V_j \in \boldsymbol{V}$, the corresponding $U_i$ and $U_j$ are independent.
In other words, no bidirected arrow exists in its induced causal diagram $(\mathcal{G})$.

\textbf{Interventions and the \textit{do}-Operator}: 
Given an SCM $\mathcal{M}$, and a set of endogenous variables $\boldsymbol{X} \subseteq \boldsymbol{V}$, an intervention $\textit{do}(\boldsymbol{X} \coloneqq \boldsymbol{x})$ corresponds to replacing the generation mechanisms $\mathcal{F}$ with $\mathcal{F}_{\boldsymbol{x}} = \{f_i : V_i \notin \boldsymbol{X}\} \cup \{\boldsymbol{X} \coloneqq \boldsymbol{x}\}$.
In words, $\mathcal{F}_{\boldsymbol{x}}$ is formed by deleting from $\mathcal{F}$ all functions $f_i$ corresponding to members of set $\boldsymbol{X}$ and replacing them with the set of constant functions $\{\boldsymbol{X} \coloneqq \boldsymbol{x}\}$.
We refer to the altered SCM by $\mathcal{M}_{\boldsymbol{x}}$, and the interventional $(\mathcal{L}_2)$ distribution of endogenous variables by $P_{\boldsymbol{V}}^{\mathcal{M}_{\boldsymbol{x}}}(\cdot)$ or in short $P_{\boldsymbol{V}_{\boldsymbol{x}}}(\cdot)$.
The interventional (or experimental) distribution helps us analyze the effect of taking actions, i.e., what would happen if we apply an intervention?

\textbf{Counterfactuals}: 
Given an SCM $\mathcal{M}$, two sets of endogenous variables $\boldsymbol{X}, \boldsymbol{E} \subseteq \boldsymbol{V}$, observed realizations $\boldsymbol{e}$ (evidence) for $\boldsymbol{E}$, and an intervention $\textit{do}(\boldsymbol{X} := \boldsymbol{x})$, the counterfactual $(\mathcal{L}_3)$ distribution $P_{\boldsymbol{V}}^{\mathcal{M}_{\boldsymbol{x}}}(\cdot|\boldsymbol{E} = \boldsymbol{e})$ or in short $P_{\boldsymbol{V}_{\boldsymbol{x}}}(\cdot|\boldsymbol{E} = \boldsymbol{e})$ corresponds to the distribution entailed by $\mathcal{M}_{\boldsymbol{x}}$ using the posterior distribution $P_{\boldsymbol{U}|\boldsymbol{E}}(\cdot|\boldsymbol{e})$ over the exogenous variables.
In case of deterministic counterfactuals ($\delta$-distribution), we refer to them as $\boldsymbol{V}_{\boldsymbol{x}}|\boldsymbol{E} = \boldsymbol{e}$.
\citet[Ch.~7]{pearl2009causality} proposes the following three-step procedure for counterfactual estimation.
i) \textit{Abduction:} Update $P_{\boldsymbol{U}}$ with $\boldsymbol{e}$ to obtain $P_{\boldsymbol{U}|\boldsymbol{E}}$.
ii) \textit{Action:} Update the SCM $\mathcal{M}$ to $\mathcal{M}_{\boldsymbol{x}}$.
iii) \textit{Prediction:} Use the updated distribution of exogenous variables and the updated SCM to estimate the counterfacual distribution.
For generalizations of this definition, e.g., to nested counterfactuals, refer to \citet{correa2021nested}.
Counterfactual distributions allow us to imagine hypothetical worlds where everything is fixed other than interventions. 

\textbf{Identifiability}:
% Evaluating causal queries given this partial state of knowledge is a subtle problem known as \emph{identification}.
% An $\mathcal{L}_i$ query is identifiable using $\mathcal{L}_j$ information if its answer can be expressed purely based on $\mathcal{L}_j$ distributions.
% This is always true if $j \geq i$.
% Characterizing conditions where this holds for $j < i$ has been subject to extensive research efforts~\cite{spirtes2001causation}.
Evaluating causal queries given a partial state of knowledge is a subtle problem. An $\mathcal{L}_i$ query is identifiable using $\mathcal{L}_j$ information if its answer can be expressed purely based on $\mathcal{L}_j$ distributions $(i,j \in \{1,2,3\})$.
Formally, let $Q(\mathcal{M})$ be an $\mathcal{L}_i$ query of an SCM $\mathcal{M}$.
In a class $\mathbb{M}$ of SCMs, $Q$ is identifiable if for any pair of SCMs $\mathcal{M}_1$ and $\mathcal{M}_2$ from $\mathbb{M}$, $Q(\mathcal{M}_1) = Q(\mathcal{M}_2)$ whenever $\mathcal{M}_1$ and $\mathcal{M}_2$ match in all $\mathcal{L}_j$ queries~\citep[def.~3.2.3]{pearl2009causality}. 
This is always true if $1 \leq i \leq j \leq 3$.
Characterizing conditions where this holds for $1\leq j < i \leq 3$ has been subject to extensive research efforts~\cite{spirtes2001causation}.

==> sections/conclusion.tex <==
\section{Concluding Remarks}
\label{sec:conclusion}

In this work, we defined Bijective Generation Mechanisms (BGM), a class of models that contain several widely used causal models in the literature (\S\ref{sec:problem}).
We established their counterfactual identifiability for three well-known causal structures (\S\ref{sec:identifiability}) and proposed a practical learning method that casts learning a BGM as structured generative modeling (\S\ref{sec:learning}).
We evaluated our methodology in a visual task and demonstrated its application to a real-world video streaming simulation task (\S\ref{sec:eval}).
Finite sample analysis of our identifiability theorems, extending the identifiable causal structures, and applications of the proposed method to real-world problems in various field, e.g., econometrics, computer systems, causal ML, etc., are exciting directions for future work.

==> sections/counterfactual.tex <==
\section{Efficient Counterfactual Estimation}
\label{sec:counterfactual}

% Assuming the optimization procedure of the structured generative networks described above converges to its global optima, we end up with the generation function of $V$ given its parents $\boldsymbol{X}$ (Green CGMs in \Cref{fig:CNF}), which is guaranteed to be equivalent to the ground truth generation mechanism according to the theoretical development of \S\ref{sec:identifiability}.

Once we have learned a BGM using the techniques in \S\ref{sec:learning}, estimating counterfactual queries is a straightforward application of the Abduction-Action-Prediction procedure (\S\ref{sec:prelim}). We illustrate this using two examples. 

Suppose we are interested in a counterfactual query $V_{\boldsymbol{x}'}|\{\boldsymbol{X} = \boldsymbol{x}, V = v\}$, which seeks to determine the necessity of causation, e.g., given that a patient recovered ($V=1$) under a treatment $X=1$, would she have also recovered without the treatment ($X=0$).  This query is in general non-identifiable from observational ($\mathcal{L}_1$) and interventional ($\mathcal{L}_2$) data~\cite{pearl1999probabilities,tian2000probabilities,li2022probabilities}.
However, if we can approximate the generation mechanism of $V$ as a BGM, and if one of the identifiability conditions of \S\ref{sec:identifiability} holds, there is hope. Specifically, we first learn the BGM from
% interventional (\S\ref{sub:Markovian})or 
observational data (\S\ref{sec:learning}). Then, we do the abduction step by inverting the BGM, i.e., $\hat{u} = \hat{f}^{-1}(\boldsymbol{x}, v)$, and  pass the counterfactual $\boldsymbol{x}'$ through the BGM to get the counterfactual estimate, i.e., $v' = \hat{f}(\boldsymbol{x'}, \hat{u})$.

As another example, consider $P(V_{\boldsymbol{x}_2}|\boldsymbol{X} = \boldsymbol{x}_1)$ which questions the effect of treatment on the treated~\cite{shpitser2009effects}.
For the abduction step, we invert the learned BGM ($\hat{f}$) for all the observed samples (e.g., patients) assigned to $\boldsymbol{x}_1$ to obtain samples of the exogenous posterior distribution $P_{\hat{U}|\boldsymbol{x}_1}$ as $\hat{u} = \hat{f}^{-1}(\boldsymbol{x}_1, v), v \sim P(V|\boldsymbol{x_1})$.
For the prediction step, we pass the samples $\hat{u}$ through the BGM with $X=\boldsymbol{x}_2$, to obtain samples of the counterfactual distribution of interest $v' = \hat{f}(\boldsymbol{x}_2, \hat{u}), \hat{u} \sim P_{\hat{U}|\boldsymbol{x}_1}$.

The examples above considered only the generation function of particular node $V \in \boldsymbol{V}$ in the causal diagram.
If all generation functions of an SCM ($\mathcal{F}$) are well-approximated by BGMs, and can also be learned in the settings described in \S\ref{sec:identifiability}, then we can answer every counterfactual query in a similar way.
However, not all generation mechanisms need to be BGMs, or known, for answering a particular counterfactual query of interest.
For instance, there is no need to learn BGMs for ancestors of the variables that we intervene on, or the variables that do not appear in the evidence and do not have dashed-bidirected edges to the evidence.

%\footnote{Conditioning on evidence changes the distribution of the exogenous variable associated with this node if such an edge exists.}

==> sections/eval.tex <==
\section{Experiments}
\label{sec:eval}

We evaluate our techniques in two settings: (i) a simple task that allows us to visualize our approach and prior baselines, and (ii) a real-world video streaming simulation task. 
\Cref{app:exp} has implementation details.

\subsection{Counterfactual Ellipse Generation}
\label{eval:ellipse}

%Cartesian and trigonometric~\cite{muller1923vorlesungen} representations of an ellipse provide an opportunity for visual evaluation of our method.
A standard ellipse is determined by two parameters: a semi-major and semi-minor axis ($a, b$).
If we further specify an angle, we get a single point on the ellipse.
Let $U \in \mathbb{R}^2$ be the two parameters of an ellipse, $X \in (0, 2\pi)$ an angle that specifies a single point, $V \in \mathbb{R}^2$ the Cartesian coordinates of this point, and $f$ the function that calculates these coordinates given $U$ and $X$.

Suppose we are given data generated as follows. We sample $z \sim P_Z$, $u \sim P_{U|Z=z}$ and $x \sim P_{X|Z=z}$, and output the data tuple $(z, x, v\coloneqq f(u,x))$. Here, $P_Z$, $P_{U|Z}$, and $P_{X|Z}$ are three predefined distributions (see \Cref{app:ellipse} for details). The important point is that conditioned on $Z$, the ellipse parameters and angles are independent $(U \indep X|Z)$, but $U$ and $X$ are not independent unconditionally. For a specific pair $(x, v)$ observed in the dataset (evidence), our goal is to draw the entire ellipse that the point $v$ belongs to. This can be done by estimating counterfactual queries, $V_{x'}|\{X=x, V=v\}$, for $x'\in (0, 2\pi)$. 

% \begin{align}
% Z &\coloneqq \epsilon_z, \; \epsilon_z \sim \text{Unif}(-0.5, 0.5)\\
% X &\coloneqq (1.44254843z + 0.59701923 + \epsilon_x) ~\%~ (2\pi), \; \epsilon_x \sim \text{Normal}(0, 1)\\
% U_0 &\coloneqq e^{1.64985274z + 0.2656131} + \epsilon_{u_0}, \; \epsilon_{u_0} \sim \text{Beta}(1, 1)\\
% U_1 &\coloneqq U_0(1 + \epsilon_{u_1}e^{1.61323358z - 0.18070237}), \; \epsilon_{u_1} \sim \text{Exponential}(1)\\
% V_0 &\coloneqq U_0\Big(2 + \sin(X)\Big)\\
% V_1 &\coloneqq U_1\Big(2 + \cos(X)\Big)\\
% \end{align}

%Suppose we are given data organized in several datasets. Each dataset provides a set of $(x,v)$ points from some ellipses with unknown parameters $U$. Let $Z$ denote the dataset identifier, and assume that in each dataset, ellipse parameters and angles are independent, i.e., $(U \indep X|Z)$. However, $U$ and $X$ are not independent when aggregating the datasets.

%Here, the dataset identifier $Z$ plays   creates a spurious correlation among them, where dataset identifier plays the role of a confounder.


%To learn $\hat{f}$, we generate data according to the causal diagram in \Cref{subfig:PGM:CNF-BC}, where $Z$ denotes the dataset identifier (alternatively, \emph{ellipse race}). In each dataset, ellipse parameters and angles are independent $(U \indep X|Z)$. However, aggregating the datasets creates an spurious correlation among them, where dataset identifier plays the role of a confounder.

This task corresponds to our \textbf{BC} setting with $Z$ as the backdoor variable. We evaluate our method for BC visually (\Cref{fig:ellipse}) and quantitatively (\Cref{table:ellipse}).
As you can see, it achieves a high accuracy as opposed to the baselines, both of which are single CGMs that do not take the causal structure into account, which is common in prior work~\cite{lample2017fader,zhu2017unpaired,he2019attgan}. 
\textbf{Baseline-x} models $P(V|X)$ and \textbf{baseline-xz} models $P(V|X, Z)$.

\begin{figure}
% \vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=0.9\linewidth]{icml2023/figures/ellipse2.png}}
\caption{BC (ours) is the only scheme that generates an ellipse.}
\label{fig:ellipse}
\vspace{-7pt}
\end{center}
% \vskip -0.2in
\end{figure}

\begin{table}[t]
\caption{Counterfactual Ellipse Generation Accuracy}
\label{table:ellipse}
% \vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{l|ccr}
\toprule
Scheme & BC & Baseline-x & Baseline-xz\\
% \midrule
MAPE & 1\% & 6607\% & 6582\% \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\end{table}

\subsection{Case Study: Video Streaming Simulation}
\label{subsec:trace-driven}

Video streaming clients use Adaptive Bitrate (ABR) algorithms to continually adapt the bitrate of a video stream based on network conditions. ABR algorithms select a bitrate for each few-second chunk of video among a finite set of available choices. These algorithms have a significant impact on user experience (e.g., video quality and stalls) and have been the subject of extensive research~\cite{tian2012towards,huang2014buffer,yin2015control,sun2016cs2p,mao2017neural,akhtar2018oboe,spiteri2020bola}. 

Trace-driven simulation is a common approach to design and evaluate ABR algorithms. Here, one collects traces from real video streaming sessions, with each trace providing a timeseries of observed network throughput (and possibly other player metrics) for every video chunk. At simulation time, the traces are replayed (to represent network behavior) while simulating the dynamics of video clients under new ABR algorithms. However, simply replaying a throughput trace can bias simulation outcomes~\cite{bartulovic2017biases, causalsim}, because changing the ABR algorithm could effect the throughput that would have been achieved for the same video streaming session. 

%\footnote{This is a widely used simulation paradigm in computer systems, called \emph{trace-driven simulation}.}



% When you watch a video, e.g., on Netflix, an Adaptive Bitrate (ABR) algorithm on your video client (running on your web browser, home TV, game console, etc.) is continuously solving an optimization problem based on its perception of the network conditions, to ensure you get a good viewing experience.
% For each video chunk, it chooses a bitrate from a finite set of available ones, to download from the video server.
% Picking low bitrates means low-quality video.
% Picking high bitrates though causes longer chunk download times which could empty the playback buffer and halt the video while waiting for the download of a new chunk.
% Both playback stall and low quality hurt the watching experience, and it is the ABR algorithm's goal to achieve a pleasant trade-off between these two conflicting objectives.
% Quality of experience has a huge causal impact on content providers' revenue~\cite{dobrian2011understanding,krishnan2012video}.
% As a result, designing good ABR algorithms for maximizing it has been subject to research for a long time~\cite{tian2012towards,huang2014buffer,yin2015control,sun2016cs2p,mao2017neural,akhtar2018oboe,spiteri2020bola}.


% A large portion of study of ABR algorithms happens in simulation, where instead of simulating both the video client and the underlying network, it is common to only simulate the video client (where the ABR algorithm lives), making it simpler, faster, and alleviating the need for detailed knowledge of the underlying network.
% To account for the effect of the network which is not simulated, it is common to collect a collection of traces from a real-world deployment of an ABR algorithm, where the trace is a time series of network throughput for the download of each video chunk.
% At simulation time, these traces are replayed (representing real networks) while simulating dynamics of video client for new ABR algorithms.\footnote{This is a widely used simulation paradigm in computer systems, called \emph{trace-driven simulation}.}

% A key assumption made when replaying a throughput trace is that changing the ABR algorithm (from the one used for trace collection to the new one we want to simulate) would not affect it, which is known to be incorrect and a key cause of bias in simulation outcomes~\cite{bartulovic2017biases}.
% In fact, the bitrates chosen by the ABR algorithm do affect the achieved throughput.

\Citet{causalsim} formulated bias removal in this type of simulation as a counterfactual estimation problem where for download of each chunk, $V$ is the achieved throughput, $X$ is the chosen bitrate,  $U$ is the unobserved bottleneck link capacity, and $V = f(U, X)$.
Note that in this problem, $f$ is strictly increasing for each value of $X$ as higher bottleneck link capacity ($U$) increases the achieved throughput ($V$).
They prove identifiability for this counterfactual query assuming data collected in a Randomized Control Trial (RCT) with sufficiently diverse ABR algorithms and low-rank structure of the underlying BGM. 
They use a deterministic auto-encoder~\cite{ghosh2019variational} equipped with adversarial learning for distribution matching for counterfactual estimation, and present experimental results (including a real-world ABR design case study) that show it significantly improves simulation accuracy compared to standard (biased) trace-driven simulators. 

Next, we demonstrate how each set of conditions for identifiability (\S\ref{sec:identifiability}) translates to this real-world problem along with the efficacy of our practical algorithm (\S\ref{sec:learning}) using the ABR simulator provided by \citet{causalsim}. We use the simulator to generate traces for each setting, which we use to learn the BGM.
The simulator gives us ground-truth counterfactuals for error calculation.
We normalize the Mean Squared Error (MSE) of our method's counterfactual estimates by the MSE of a standard (biased) video streaming simulator that assumes chosen bitrates do not affect the achieved throughput.
All results are in \Cref{table:abr} with mean and standard deviation calculated over ten random seeds trained until training loss convergence.
%\footnote{\label{foot:converge}Excluding few outliers whose training does not converge.}

\begin{table}
\caption{Counterfactual estimation accuracy of different schemes and their training time for video streaming simulation}
\label{table:abr}
% \vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcr}
\toprule
Scheme & Normalized MSE $(\%)$ & Time ($s$) \\
\midrule
Markovian    & \; 4.1 $\pm$ 2.1& \; \; 28 $\pm$ 0\\
IV    & 10.0 $\pm$ 0.7& \; 127 $\pm$ 1\\
CausalSim    & \; 9.3 $\pm$ 1.0& 1091 $\pm$ 1\\
% BC-BBA    & 16.1 $\pm$ 7.3& \; \; 45 $\pm$ 1\\
% BC-BOLA    & \; 4.6 $\pm$ 0.9& \; \; 30 $\pm$ 0\\
BC    & 10.4 $\pm$ 7.8& \; \; 37 $\pm$ 8\\
IV+BC    & \; 6.4 $\pm$ 2.4& \; \; 49 $\pm$ 1\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\end{table}

\textbf{The Markovian Case}:
The causal structure in this problem is not Markovian because $X$ (chosen bitrate) and $V$ (observed throughput) are both affected by underlying network conditions (latent confounder). 
However, we can remove the confounding effect if the ABR algorithm used for trace collection chooses random bitrates from time to time, and we only select the subset of traces with these random decisions as $\mathcal{D}$ (\Cref{fig:causal-dag}).
This scheme achieves the lowest error in Table~\ref{table:abr} as it has access to the most pristine data (perfect confounding removal by invasive randomization).

\textbf{Instrumental Variable (IV)}:
It is common for video service providers to conduct RCTs over various ABR algorithms for their comparison.
If traces are collected from an RCT, their causal structure naturally fits \Cref{subfig:IV} where IV ($I$) is the algorithm identifier.
This is the same setting that \textbf{CausalSim}~\yrcite{causalsim} explores, so we use their adversarial learning method as a baseline.
We collect RCT data over ten different provided algorithms.
Our IV method achieves almost the same accuracy as CausalSim (slight difference is not statistically significant), but converges $8.6 \times$ faster since it does not require bi-level (adversarial) optimization.

\textbf{Backdoor Criterion (BC)}:
Buffer based ABR algorithms are those that only make use of the client's current playback buffer level to make bitrate decisions.
They are strong ABR algorithms despite their simplicity and are widely used in practice~\cite{yan2020learning}.
If a trace is collected using a buffer based algorithm (and includes playback buffer observations), the causal structure follows \Cref{subfig:BC} where $Z$ is the buffer used for choosing the bitrate. Hence, it satisfies the backdoor criterion. Table~\ref{table:abr} shows that our BC method applied to buffer-based traces is quite accurate even without access to RCT data (although it is slightly worse than CausalSim and IV). 

% We have two different buffer based algorithm implementations, BBA and BOLA, whose traces we use to learn BGMs called \textbf{BBA-BC} and \textbf{BOLA-BC}.
% Although this trace collection method is much less invasive than running an RCT, BOLA-BC beats IV schemes that require an RCT.
% BBA-BC, although decreases the baseline error almost by a factor of 6, is less accurate than BOLA-BC.
% We believe this difference is due to some intrinsic difference between the two ABR algorithms.
% Characterization and design of performant algorithms that are suitable for trace collection is an interesting direction which we leave for the future.
% \todo{Combine results and remove this paragraph to save space?}

\textbf{IV + BC}:
It is possible to combine settings explored in \S\ref{sec:identifiability} to further improve accuracy provided the problem has the appropriate causal structure. For example, in video streaming simulation, if $\mathcal{D}$ is collected in an RCT over buffer based algorithms, the BC and IV cases apply simultaneously. We refer to this case as IV+BC. 
Similar to the IV case, the algorithm identifier is the instrumental variable while the tuple (algorithm identifier, buffer) satisfies the backdoor criterion. \Cref{app:video:IV+BC} describes the structured generative network for this case. We apply it to traces collected using an RCT over two buffer based algorithms. 
IV+BC decreases the average error compared to the BC scheme by almost $38\%$.

==> sections/identifiability.tex <==
\section{Identifiability}
\label{sec:identifiability}

\begin{figure}
    \centering
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=0.6\linewidth]{icml2023/figures/sub-graph.pdf}
        \caption{Non-Markovian}
        \label{subfig:sub-graph}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=0.6\linewidth]{icml2023/figures/intervened.pdf}
        \caption{Markovian}
        \label{subfig:intervened}
    \end{subfigure}
    \caption{Causal diagram $\mathcal{G}$'s sub-graph related to generation of $V$}
    \label{fig:causal-dag}
\end{figure}

Without loss of generality, we focus on identifying the generation mechanism $f_i$ of a particular endogenous node $V_i$ shown in \Cref{eqn:generation_mechanism}.
For ease of exposition, we drop the subscript $i$, and refer to $\text{Pa}(V)$ as $\boldsymbol{X}$.
The sub-graph of $\mathcal{G}$ which is related to the generation of $V$ is depicted in \Cref{subfig:sub-graph}.
The dashed-bidirected arrow indicates potential existence of an unobserved confounder.
All proofs are in \Cref{app:proof}.

% We now provide three sets of constraints on $\hat{f}$ and $f_{\star}$ which imply their equivalence. 
% We motivate each constraint set with a causal structure. Importantly, the required constraints on $\hat{f}$ can be verified from observed data $\mathcal{D}$, which leads to a tractable procedure to learn $\hat{f}$.  

\edited{We provide three sets of constraints on $f$ and the underlying causal structure that imply counterfactual identifiability given an observed ($\mathcal{L}_1$) data distribution ($\mathcal{D}$), i.e., given $\mathcal{D}$, each set of constraints identifies $f$ up to indeterminacies that do not affect counterfactual queries.}
% We motivate each constraint set with a causal structure. 

$U$ and $V$ can be single- or multi-dimensional \edited{in general}. Our results in \S\ref{sub:Markovian} and \S\ref{sub:IV} are for the scalar case, while the result in \S\ref{sub:BC} applies to multi-dimensional  $U$ and $V$.

%Each set of constraints provides a criteria for counterfactual identifiability. Specifically, if the true (unknown) generation mechanism $f$ and an estimated one $\hat{f}$ satisfy the constraints, then $\hat{f}$ produces an equivalent BGM to $f$, establishing counterfactual identifiability. As we will see, the constraints also provide constructive identifiablity in each 

\subsection{The Markovian Case}
\label{sub:Markovian}
If the exogenous variable $U$ associated with $V$ is \edited{independent of} its parents $\boldsymbol{X}$, we end up with the causal diagram shown in \Cref{subfig:intervened} where $\boldsymbol{X} \indep U$.\footnote{It is common practice to exclude the exogenous variable $U$ from the causal diagram.}

%, or if they are \edited{dependent} but we have access to interventional $(\mathcal{L}_2)$ data from an experiment where we intervene on $X$ to break the \edited{dependence},

% \begin{theorem}
% \label{thm:intervention}
% BGMs $f_{\star}$ and $\hat{f}$ are equivalent in $\mathcal{D}$ if
% \begin{enumerate}
%     \item (Markovian) $U^{\star} \indep \boldsymbol{X}$ and $\hat{U} \indep \boldsymbol{X}$.
%     \item $\forall \boldsymbol{x}: f_{\star}(\boldsymbol{x}, \cdot)$ and $\hat{f}(\boldsymbol{x}, \cdot)$ are both strictly increasing.\footnote{See \Cref{app:proof} for a generalization of this condition.\label{foot-precise}}
%     % \item $U, \hat{U}, V$ are single-dimensional. \todo{Implied from the previous condition?}
% \end{enumerate}
% \end{theorem}
\edited{
\begin{theorem}
\label{thm:intervention}
BGM $f$ is counterfactually identifiable given $P_{\boldsymbol{X}, V}$ if
\begin{enumerate}
    \item (Markovian) $U \indep \boldsymbol{X}$.
    \item For all $\boldsymbol{x}$, $f(\boldsymbol{x}, \cdot)$ is either a strictly increasing function or a strictly decreasing function.
\end{enumerate}
\end{theorem}
}
This theorem is similar to \citet[Thm.~1]{lu2020sample}, and is mentioned here for completeness. In this result, \edited{$U, \boldsymbol{X}, V$} can be discrete or continuous. 
Note that 
% the monotonicity assumption is necessary \,---\, 
independence of $U$ and $\boldsymbol{X}$ \edited{by itself} is not sufficient for \edited{identifiability} as demonstrated with a counter-example in \Cref{app:subsub:counter-example} and an experiment in \Cref{app:ellipse:failure}.
It is not clear how to generalize the monotonicity condition to BGMs with multi-dimensional $V$, which is a known issue in Markovain causal structures~\cite{non-ident}.

\subsection{Instrumental Variable (IV)}
\label{sub:IV}
\begin{figure}
    \centering
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=0.6\linewidth]{icml2023/figures/IV.pdf}
        \caption{Instrumental Variable}
        \label{subfig:IV}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=0.6\linewidth]{icml2023/figures/BC.pdf}
        \caption{Backdoor Criterion}
        \label{subfig:BC}
    \end{subfigure}
    \caption{Instrumental Variable and Backdoor Criterion examples.}
\end{figure}
Even with an unobserved confounder, we can establish \edited{counterfactual identifiability} from observational $(\mathcal{L}_1)$ data if we can find IVs relative to the pair $(\boldsymbol{X}, V)$. We define an IV as a set of variables independent of $U$ that affect $V$ only through $\boldsymbol{X}$.
\Cref{subfig:IV} shows an example in which $\boldsymbol{I}$ is an IV with respect to $(\boldsymbol{X}, V)$.\footnote{There are several other IV definitions in the causal literature that capture the same concept, e.g., \citet{bowden1990instrumental,pearl1995testability,angrist1996identification,heckman1999local}.
See \citet[Sec.~7.4.5]{pearl2009causality} for a discussion.}
% What we mean by an IV is a set of variables independent of $U$, and not independent of $\boldsymbol{X}$.

The following theorem formalizes \edited{counterfactual identifiability} in this setting for discrete-valued $\boldsymbol{X}$ and $\boldsymbol{I}$, i.e., $\boldsymbol{X} \in \mathbb{X} \triangleq \{\boldsymbol{x}_1, \ldots, \boldsymbol{x}_n\}$ and $\boldsymbol{I} \in \mathbb{I} \triangleq \{\boldsymbol{i}_1, \ldots, \boldsymbol{i}_n\}$.\footnote{If $|\mathbb{I}| > n$, pick any subset with $n$ members.}

% \begin{theorem}
% \label{thm:IV}
% BGMs $f_{\star}$ and $\hat{f}$ are equivalent in $\mathcal{D}$ if
% \begin{enumerate}
%     \item (IV) $\boldsymbol{I} \indep U^{\star}$ and $\boldsymbol{I} \indep \hat{U}$.
%     \item $\forall \boldsymbol{x} \in \mathbb{X}: f_{\star}(\boldsymbol{x}, \cdot)$ and $\hat{f}^{-1}(\boldsymbol{x}, \cdot)$ are strictly increasing\footref{foot-precise} and two times differentiable functions.
%     \item $P_{\hat{U}}(\cdot)$ is differentiable.
%     \item $P(\boldsymbol{i}, \boldsymbol{x}, \cdot)$ is differentiable for every $\boldsymbol{i}, \boldsymbol{x}, u^{\star}$.
%     % \item $U \in \mathbb{U}$ is continuous and single-dimensional.
%     \item (Positivity) $\forall u^{\star}, \hat{u}, \boldsymbol{x} \in \mathbb{X}: P_{U^{\star}, \boldsymbol{X}}(u^{\star}, \boldsymbol{x}) > 0$ and $P_{\hat{U}, \boldsymbol{X}}(\hat{u}, \boldsymbol{x}) > 0$.
%     \item (Variability) $\forall u^{\star}: |\det \boldsymbol{M}(u^{\star}, \mathbb{I})| \ge c > 0$ , where 
%     \begin{equation*}
%     \boldsymbol{M}(u^{\star}, \mathbb{I}) \triangleq    
%     \begin{bsmallmatrix}
%     P(\boldsymbol{x}_1|u^{\star},\boldsymbol{i}_1) & \ldots & P(\boldsymbol{x}_n|u^{\star},\boldsymbol{i}_1) \\
%     \vdots                   & \ddots & \vdots                   \\
%     P(\boldsymbol{x}_1|u^{\star},\boldsymbol{i}_n) & \ldots & P(\boldsymbol{x}_n|u^{\star},\boldsymbol{i}_n) \\
%     \end{bsmallmatrix}
%     \end{equation*}
% \end{enumerate}
% \end{theorem}

\edited{
\begin{theorem}
\label{thm:IV}
BGM $f$ is counterfactually identifiable given $P_{\boldsymbol{X}, V, \boldsymbol{I}}$ if
\begin{enumerate}
    \item (IV) $\boldsymbol{I} \indep U$.
    \item For all $\boldsymbol{x} \in \mathbb{X}$, $f(\boldsymbol{x}, \cdot)$ and $f^{-1}(\boldsymbol{x}, \cdot)$ are either strictly increasing or strictly decreasing, and two times differentiable functions.
    \item $P(\boldsymbol{i}, \boldsymbol{x}, \cdot)$ is differentiable for every $\boldsymbol{i} \in \mathbb{I}, \boldsymbol{x} \in \mathbb{X}$.%$, u$.
    % \item $U \in \mathbb{U}$ is continuous and single-dimensional.
    \item (Positivity) $\forall u, \boldsymbol{x} \in \mathbb{X}: P_{U, \boldsymbol{X}}(u, \boldsymbol{x}) > 0$.
    \item (Variability) $\forall u: |\det \boldsymbol{M}(u, \mathbb{I})| \ge c > 0$ , where 
    \begin{equation*}
    \boldsymbol{M}(u, \mathbb{I}) \triangleq    
    \begin{bsmallmatrix}
    P(\boldsymbol{x}_1|u,\boldsymbol{i}_1) & \ldots & P(\boldsymbol{x}_n|u,\boldsymbol{i}_1) \\
    \vdots                   & \ddots & \vdots                   \\
    P(\boldsymbol{x}_1|u,\boldsymbol{i}_n) & \ldots & P(\boldsymbol{x}_n|u,\boldsymbol{i}_n) \\
    \end{bsmallmatrix}
    \end{equation*}
\end{enumerate}
\end{theorem}
}

Besides the technical conditions required for the proof, the variability condition in \Cref{thm:IV} has the following interpretation: the IV must take a sufficient number of distinct values (at least as many values as possible for $\boldsymbol{X}$), and that the IV must have a strong influence on $\boldsymbol{X}$. Positivity implies that the support of U is independent of $\boldsymbol{X}$.

\subsection{The Backdoor Criterion (BC)}
\label{sub:BC}
The second setting in which we can establish counterfactual identifiability from observational $(\mathcal{L}_1)$ data in the presence of latent confounding is when there exists a set of variables $(\boldsymbol{Z})$ that satisfy the backdoor criterion (BC) with respect to $(\boldsymbol{X}, V)$, i.e., if $\boldsymbol{Z}$ blocks every path between $\boldsymbol{X}$ and $V$ that contains an arrow into $\boldsymbol{X}$.\footnote{\citet[Def.~3.3.1]{pearl2009causality} requires $\boldsymbol{Z}$ to be non-descendent of $\boldsymbol{X}$ as well, but we do not need such a requirement as our goal is not to use $\boldsymbol{Z}$ for adjustment.}
Intuitively, we want $\boldsymbol{Z}$ to be responsible for all the spurious correlation (the dashed-bidirected edge) between $\boldsymbol{X}$ and $U$.
\Cref{subfig:BC} demonstrates an example where $\boldsymbol{Z}$ satisfies the BC with respect to $(\boldsymbol{X}, V)$. 

In the following, assume $U, V \in \mathbb{R}^d$.

% \begin{theorem}
% \label{thm:BC}
% BGMs $f_{\star}$ and $\hat{f}$ are equivalent in $\mathcal{D}$ if
% \begin{enumerate}
%     \item (BC) $U^{\star} \indep \boldsymbol{X} | \boldsymbol{Z}$ and $\hat{U} \indep \boldsymbol{X} | \boldsymbol{Z}$.
%     \item  $\forall \boldsymbol{x}: \nabla_{\boldsymbol{x}}|\det\boldsymbol{J}_{f_{\star}(\boldsymbol{X}, \cdot)}|$ and $\nabla_{\boldsymbol{x}}|\det\boldsymbol{J}_{\hat{f}^{-1}(\boldsymbol{X}, \cdot)}|$ exist.
%     % \item For every $\boldsymbol{x}, v: \nabla_{\boldsymbol{x}} f_{\star}^{-1}(\boldsymbol{x}, v), \nabla_{\boldsymbol{x}}\nabla_v f_{\star}^{-1}(\boldsymbol{x}, v)$ exist and $|\det \boldsymbol{J}_{f_{\star}^{-1}(\boldsymbol{x}, \cdot)}| > 0$.
%     % \item  For every $\boldsymbol{x}, \hat{u}: \nabla_{\boldsymbol{x}} \hat{f}(\boldsymbol{x}, \hat{u}), \nabla_{\boldsymbol{x}}\nabla_{\hat{u}} \hat{f}(\boldsymbol{x}, \hat{u})$ exist and $|\det \boldsymbol{J}_{\hat{f}(\boldsymbol{x}, \cdot)}| > 0$.
%     % \item $\forall \boldsymbol{x}, u, v: \nabla_{\boldsymbol{x}} \hat{f}(\boldsymbol{x}, u)$ and $\nabla_{\boldsymbol{x}} f^{-1}(\boldsymbol{x}, v)$ exist.
%     % \item $\forall \boldsymbol{x}, u, v: \nabla_{\boldsymbol{x}}\nabla_u \hat{f}(\boldsymbol{x}, u)$ and $\nabla_{\boldsymbol{x}}\nabla_v f^{-1}(\boldsymbol{x}, v)$ exist.
%     % % \item $P_{U|\boldsymbol{Z}}(\cdot|\boldsymbol{z})$ is differentiable for every $\boldsymbol{z}$.
%     % \item $\forall \boldsymbol{x}, u: |\det \boldsymbol{J}_{f^{-1}(\boldsymbol{x}, \cdot)}| > 0, \; |\det \boldsymbol{J}_{\hat{f}(\boldsymbol{x}, \cdot)}| > 0$.
%     \item (Variability) $\forall u^{\star}:$ Instances $\boldsymbol{z}_1, \ldots, \boldsymbol{z}_{d+1}$ exist such that $|\det \boldsymbol{M}(u^{\star}, \boldsymbol{z}_1, \ldots, \boldsymbol{z}_{d+1})| > 0,$ where
%     \begin{equation*}
%     \small{\boldsymbol{M}(u^{\star}, \boldsymbol{z}_1, \ldots, \boldsymbol{z}_{d+1})} \triangleq    
%     \begin{bsmallmatrix}
%     P(u^{\star}|\boldsymbol{z}_1) & \nabla_{u^{\star}}P(u^{\star}|\boldsymbol{z}_1)\\
%     \vdots                & \vdots                 \\
%     P(u^{\star}|\boldsymbol{z}_{d+1}) & \nabla_{u^{\star}}P(u^{\star}|\boldsymbol{z}_{d+1})\\
%     \end{bsmallmatrix}
%     \end{equation*}
% \end{enumerate}
% \end{theorem}

\edited{
\begin{theorem}
\label{thm:BC}
BGM $f$ is counterfactually identifiable given $P_{\boldsymbol{X}, V, \boldsymbol{Z}}$ if
\begin{enumerate}
    \item (BC) $U \indep \boldsymbol{X} | \boldsymbol{Z}$.
    \item  $\forall \boldsymbol{x}: \nabla_{\boldsymbol{x}}|\det\boldsymbol{J}_{f(\boldsymbol{x}, \cdot)}|$ and $\nabla_{\boldsymbol{x}}|\det\boldsymbol{J}_{f^{-1}(\boldsymbol{x}, \cdot)}|$ exist.
    \item (Variability) $\forall u:$ Instances $\boldsymbol{z}_1, \ldots, \boldsymbol{z}_{d+1}$ exist such that $|\det \boldsymbol{M}(u, \boldsymbol{z}_1, \ldots, \boldsymbol{z}_{d+1})| > 0,$ where
    \begin{equation*}
    \small{\boldsymbol{M}(u, \boldsymbol{z}_1, \ldots, \boldsymbol{z}_{d+1})} \triangleq    
    \begin{bsmallmatrix}
    P(u|\boldsymbol{z}_1) & \nabla_u P(u|\boldsymbol{z}_1)\\
    \vdots                & \vdots                 \\
    P(u|\boldsymbol{z}_{d+1}) & \nabla_u P(u|\boldsymbol{z}_{d+1})\\
    \end{bsmallmatrix}
    \end{equation*}
\end{enumerate}
\end{theorem}
}
In the above theorem, $\boldsymbol{Z}$ can be both discrete or continuous. The variability condition implies that $\mathbf{Z}$ must have a strong enough influence on $U$. 


%\subsection{Constructive Identifiability}
%\label{sub:constructive-identifiability}

% \begin{theorem}
% \label{thm:constructive-identifiability}
% For every set of constraints in \Cref{thm:intervention,thm:IV,thm:BC}, if we find an $\hat{f}$ that satisfies all the corresponding conditions, it is guaranteed to produce correct counterfactual estimates assuming access to sufficiently many samples from $\mathcal{D}$ and that the ground-truth BGM satisfies the conditions for $f_{\star}$. \todo{Needs a smoother statement}
% \end{theorem}

% \begin{theorem}
% \label{thm:constructive-identifiability}
% For every set of constraints in \Cref{thm:intervention,thm:IV,thm:BC}, in problems where the ground-truth BGM satisfies the conditions for $f_{\star}$, finding an $\hat{f}$ that satisfies all the corresponding conditions implies identifiability of counterfactuals from $\mathcal{D}$. \todo{Needs a smoother statement}
% \end{theorem}

% \begin{theorem}
% \label{thm:constructive-identifiability}
% For every set of constraints in \Cref{thm:intervention,thm:IV,thm:BC}, assuming that ground-truth BGM satisfies the conditions for $f_{\star}$, finding an $\hat{f}$ that satisfies all the corresponding conditions implies identifiability of counterfactuals from $\mathcal{D}$. \todo{Needs a smoother statement}
% \end{theorem}

% In the rest of this section, we follow a simple strategy by characterizing sets of constraints on $f_{\star}, \hat{f}, U^{\star}, \hat{U}$ which imply $g$-equivalence of $f_{\star}$ and $\hat{f}$.
% Let us denote the ground truth BGM and the corresponding exogenous variables by $f_{\star}$ and $U^{\star}$, respectively, assuming they satisfy the constraints.
% This implies that the proposed constraints on $\hat{f}, \hat{U}$ are a valid optimization goal for learning the BGM, as the global optima of this optimization $\hat{f}$ is $g$-equivalent to $f_{\star}$ which means they will result in the same counterfactuals (\Cref{prop:counterfactual-equivalence}).
% We refer to this property as \emph{$g$-identifiability}.
% This implies that if we find a BGM $\hat{f}$ that fits the distribution (and satisfies the constraints), it is guaranteed to be in the $g$-equivalence class of the ground truth BGM $f$, which according to \Cref{prop:counterfactual-equivalence} means that we can use it for estimating provably correct counterfactual quantities.
% We define this property as \emph{$g$-identifiability}.

% The reason we cannot recover the exact BGM $f_{\star}$, and are restricted to its $g$-equivalence class is partly because we do not know the prior distribution over the exogenous variable.
% As a result, we can get a different member of the $g$-equivalence class for each choice of the prior distribution.
% However, this is harmless because all members of this class produce correct counterfactual estimates which is our ultimate goal.

% \Cref{thm:constructive-identifiability} equips us with a tractable optimization goal for learning a BGM that is as good as the ground-truth one for counterfactual estimation assuming we are able to find the global optimum.
% % and access to the distribution $\mathcal{D}$.
% The next section provides a recipe for efficiently solving this optimization problem.

==> sections/intro.tex <==
\section{Introduction}
\label{sec:intro}

\stepcounter{footnote}
\emph{Had Cleopatra's nose been shorter, the whole face of \\the world would have changed.\footnote{Taken from \citet[Ch.~8]{pearl2018book}} (Blaise Pascal, 1669)}
\smallskip

The \emph{ladder of causation} presented by Pearl~\yrcite{pearl2018book} consists of three distinct layers encoding different types of concepts: \emph{associational}~($\mathcal{L}_1$), \emph{interventional}~($\mathcal{L}_2$), and \emph{counterfactual}~($\mathcal{L}_3$), roughly corresponding to \emph{seeing}, \emph{doing}, and \emph{imagining}, respectively.
$\mathcal{L}_1$ deals with passively observed factual information, for instance, the probability of recovery in patients who take Aspirin.
$\mathcal{L}_2$ deals with active interventions or the effect of actions, for example, what percentage of patients would recover if we give them Aspirin?
$\mathcal{L}_3$ deals with alternative ways the world could have been including ways that might conflict with how the world currently is, e.g., if the patient took Aspirin and was cured, would the headache still be gone had they not taken Aspirin?
The three levels are distinct in the sense that it is generally not possible to uniquely answer higher level queries from lower level information~\citep[Thm.~27]{bareinboim2022pearl}.
In particular, although we can determine $\mathcal{L}_2$ information by conducting experiments and actively intervening in the world, we cannot answer $\mathcal{L}_3$ questions in general, even with experiments.
In other words, they may be \emph{non-identifiable}~\cite{ibeling2020probabilistic}, or underspecified~\cite{d2020underspecification}.

Nevertheless, counterfactual queries of the form ``\emph{why--?}" and ``\emph{what if--?}" are useful in defining fundamental concepts such as harm~\cite{2022counterfactual-harm}, fairness~\cite{2017counterfactual-fairness,zhang2018fairness}, credit~\cite{2021counterfactual-credit-assignment}, regret, and blame.
They also have applications in engineering, e.g., root cause analysis~\cite{2022sage,2022causal-rootcause}, trace-driven simulation~\cite{causalsim,bothra2022veritas}, and sample efficient reinforcement learning~\cite{lu2020sample,agarwal2021persim}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this paper, we introduce a new class of causal models called \emph{Bijective Generation Mechanisms (BGM)}.
BGMs subsume several model classes studied in the literature, e.g., Nonlinear Additive Noise Models (ANM)~\cite{hoyer2008nonlinear}, Location Scale Noise Models (LSNM)~\cite{immer2022identifiability}, and post-nonlinear causal models (PNL)~\cite{zhang2009identifiability} (\S\ref{sec:problem}).
%
%For the first time, we prove counterfactual identifiability of BGMs in three popular causal structures
We establish counterfactual identifiability of BGMs for three meaningful causal structures
(\S\ref{sec:identifiability}), assuming a coarse knowledge of the underlying system in the form of a causal diagram.


Our identifiability results specify tractable criteria for finding the underlying BGM (up to equivalence, see \Cref{def:g-equivalence}), enabling counterfactual estimation.
%Previous version: , up to harmless indeterminacies (\Cref{def:g-equivalence}) for counterfactual estimation.
%Arash's suggested version: up to indeterminacies that do not affect counterfactual estimates.
We cast the search for a BGM that satisfies the specified criteria as density estimation with \emph{structured generative networks} (\S\ref{sec:learning}), which has been widely studied in the
%deep
learning literature~\cite{kingma2013auto,goodfellow2014generative,dinh2016density,arjovsky2017wasserstein,song2019generative,ho2020denoising}. 

Once the underlying BGM is learned, we use it for efficient counterfactual estimation with guarantees (\S\ref{sec:counterfactual}).
This is in contrast to symbolic counterfactual identification methods ~\cite{shpitser2007counterfactuals,correa2021nested} which express identifiable counterfactual queries in terms of interventional and observational distributions, statements that may not be computationally tractable. Furthermore, our work advances the growing literature on applying machine learning methods for counterfactual estimation. Unlike most prior work in this space that foregoes identifiability analysis~\cite{pawlowski2020deep,sanchez2021diffusion}, except in certain restricted settings (e.g., discrete domains~\cite{shalit2017estimating,oberst2019counterfactual} or absence of unobserved confounders~\cite{khemakhem2021causal,sanchez2021vaca}), our results support continuous variables, allow unobserved confounders, and extend to a more general class of generation mechanisms. 

%and also by generalizing the class of causal models they consider such as Nonlinear ANMs and LSNMs~\cite{hartford2017deep,geffner2022deep}.

We validate our techniques using a visual task (\S\ref{eval:ellipse}) and demonstrate their application to a real-world system simulation task (\S\ref{subsec:trace-driven}).
Our code is available in \href{github.com/counterfactual-BGM/cf2}{github.com/counterfactual-BGM/cf2}. This work does not raise any negative societal impacts. 





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% In this work, we focus on tractable counterfactual estimation assuming a known causal structure in the form of a causal DAG which may include unobserved confounders.
% \todo{Add Bijective Generation Mechanisms (\S\ref{sec:problem})}
% We show that causal generation mechanisms that satisfy some conditions, and the corresponding exogenous variables are identifiable up to harmless indeterminacies (\Cref{def:g-equivalence}) in three cases, using observational (\S\ref{sub:IV}, \S\ref{sub:BC}) and interventional (\S\ref{sub:Markovian}) data.
% In all cases, we construct structured generative networks~\cite{sohn2015learning} using conditional generative models (CGM) which provably learn the underlying generation mechanisms (\S\ref{sec:learning}).
% We verify our theorems and algorithms with experiments (\S\ref{sec:eval}) and show their application to the real-world problem of Video Streaming simulation (\S\ref{subsec:trace-driven}).

==> sections/learning.tex <==
\section{Efficient Learning of the BGM}
\label{sec:learning}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% In the previous section (\S\ref{sec:identifiability}), we demonstrated three different settings in which BGMs are identifiable (up to indeterminacies that are harmless for counterfactual estimation) from distribution of observed variables.
% This suggests the use of these constraints as optimization goals for learning BGMs, for which we present an efficient method in this section.

\edited{

Given an observed data distribution ($\mathcal{D}$), our goal in this section is to find a BGM $\hat{f}$ that is counterfactually equivalent to the BGM \edited{$f$} underlying the data. First, we formalize the notion of equivalence:

\begin{definition}
\label{def:g-equivalence}
\textit{(Equivalence)}
BGMs $f_1$ and $f_2$ are equivalent iff there exists an invertible function $g(\cdot)$ such that
\begin{align}
\label{eqn:g-equivalence}
    \forall \boldsymbol{x},v:& f_1^{-1}(\boldsymbol{x}, v) = g\Big(f_2^{-1}(\boldsymbol{x}, v)\Big)\text{ or alternatively}\\
\label{eqn:reverse-g-equivalence}
    \forall \boldsymbol{x},u:& f_1(\boldsymbol{x}, u) = f_2\Big(\boldsymbol{x}, g^{-1}(u)\Big).
\end{align}
\end{definition}

\begin{proposition}
\label{prop:counterfactual-equivalence}
BGMs $f_1$ and $f_2$ produce the same counterfactuals iff they are equivalent.
% \begin{proof}
% \Cref{app:proof:prop:counterfactual-equivalence}.
% \end{proof}
\end{proposition}

If we find an $\hat{f}$ which is equivalent to the BGM \edited{$f$} underlying the data, we can perform Abduction-Action-Prediction (\S\ref{sec:prelim}) using $\hat{f}$ to estimate any counterfactual quantity, which is guaranteed to produce the same counterfactuals as the true BGM \edited{$f$} via Proposition~\ref{prop:counterfactual-equivalence}.

The theorems in \S\ref{sec:identifiability} (see also the lemmas in \Cref{app:sub:lemmas}) provide a tractable objective for learning a BGM that is equivalent to the ground-truth BGM for counterfactual estimation. 
% and access to the distribution $\mathcal{D}$.
We now describe a recipe for efficiently solving this learning problem.

%For $(\boldsymbol{X}, V) \sim \mathcal{D}$, define the random variable
%\begin{equation}
%    \hat{U} \triangleq \hat{f}^{-1}(\boldsymbol{X}, V).
%\end{equation}
}

To represent the search space for $\hat{f}$, we use parameterized bijective transforms $\hat{f}_{\theta}(\boldsymbol{x}, \cdot)$ from $\hat{U}$ to $V$, conditioned on $\boldsymbol{X}$.
This resembles transforms used in Conditional Generative Models (CGM).
Furthermore, we require certain constraints on $\hat{f}_{\theta}$ depending on the case, e.g., being strictly monotonic or differentiable, which we take into account to select an appropriate model family and parameterization. For example, both the IV and BC cases require differentiablity of the transform. Conditional Normalizing Flow (CNF)~\cite{papamakarios2021normalizing} models are a good candidate for learning such functions as they are typically built using differentiable mappings with differentiable inverses (diffeomorphisms). Although our approach is applicable to any CGM with the desired properties, we use CNFs in our experiments. Appendix~\ref{app:NF} discusses CNFs in more detail. 

% As explained in \S\ref{sec:prelim}, conditional transforms utilized in CNFs are diffeomorphism, and hence viable solutions.\footnote{CNFs typically utilize transforms with efficient Jacobian for tractable likelihood computation, which could lead to large depths for a reasonable expressive power~\cite{kong2020expressive}.
% We, on the other hand, are not limited to transforms with efficient Jacobian~\cite{behrmann2019invertible,si2021autoregressive}.}
%for modeling the conditional distribution $P(V|\boldsymbol{x})$.
% CGMs model the target conditional distribution by starting from $U$ sampled from a tractable distribution, e.g., Gaussian, and optimize conditional transform's parameters in order for their output samples to match the target conditional distribution. 

Each set of constraints has an important distributional requirement (the first condition) in the form of (conditional) independence among $\hat{U}$ (\Cref{eqn:reverse_generation_mechanism}) and other variables. One way to guide the learning to attain such conditional independence properties is to use adversarial learning for distribution matching~\cite{li2017alice}.
However, a more elegant solution emerges from flipping the problem.
Instead of passing $(\mathbf{X},V) \in \mathcal{D}$ samples through $\hat{f}_{\theta}^{-1}$ (\Cref{eqn:reverse_generation_mechanism}) and optimizing the transform to satisfy the (conditional) independence, we can sample $\hat{U}$ in a way that satisfies the (conditional) independence needed in each case, and optimize $\hat{f}_{\theta}$ (\cref{eqn:generation_mechanism}) to produce  the observed conditional distribution $P_{\mathcal{D}}(V|\boldsymbol{X})$.
This has two benefits: i) (Conditional) independence is guaranteed by construction. ii) Training objective simply becomes density modeling, which has been greatly studied in the literature.

\textbf{The Markovian Case} in \S\ref{sub:Markovian} provides a simple example to  explain the learning method.
We use a strictly increasing conditional transformation as the search space for $\hat{f}_{\theta}$.
We sample $\hat{U}$ and $\boldsymbol{X}$ independently from a Gaussian distribution and the dataset $\mathcal{D}$, respectively.
This guarantees the first condition of \Cref{thm:intervention}.
We optimize the parameters of $\hat{f}_{\theta}$ to match the conditional distribution $P_{\mathcal{D}}(V|\boldsymbol{X})$.
In doing so, we are free to choose from a diverse set of objectives provided by years of research in generative modeling~\cite{mohamed2016learning}, for instance, variational loss~\cite{kingma2013auto}, adversarial loss~\cite{goodfellow2014generative}, likelihood maximization~\cite{papamakarios2021normalizing}, score matching~\cite{song2019generative} or denoising diffusion~\cite{ho2020denoising}, etc.
% Assuming perfect optimization, once training converges, the solution is guaranteed to satisfy all conditions provided in \Cref{thm:intervention}, and can be further utilized for counterfactual estimation with guarantees.

% \begin{figure}
%     \centering
%     \begin{subfigure}{0.37\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{icml2023/figures/PGM-CNF-IV.pdf}
%         \caption{Instrumental Variable}
%         \label{subfig:PGM:CNF-IV}
%     \end{subfigure}
%     \begin{subfigure}{0.37\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{icml2023/figures/PGM-CNF-BC.pdf}
%         \caption{Backdoor Criterion}
%         \label{subfig:PGM:CNF-BC}
%     \end{subfigure}
%     \caption{Graphical models for structured generative networks.}
%     \label{fig:CNF-DGM}
% \end{figure}

\begin{figure}
    \centering
    % \begin{subfigure}{0.27\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{icml2023/figures/CNF-Markovian.pdf}
    %     \vspace{-11pt}
    %     \caption{\scriptsize Markovian Case}
    %     \label{subfig:CNF-Markovian}
    % \end{subfigure}
        \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=0.6\linewidth]{icml2023/figures/PGM-CNF-IV.pdf}
        \caption{Instrumental Variable}
        \label{subfig:PGM:CNF-IV}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=0.6\linewidth]{icml2023/figures/PGM-CNF-BC.pdf}
        \caption{Backdoor Criterion}
        \label{subfig:PGM:CNF-BC}
    \end{subfigure}
    \label{fig:CNF-DGM}

    
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{icml2023/figures/CNF-IV.pdf}
        \caption{Instrumental Variable}
        \label{subfig:CNF-IV}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{icml2023/figures/CNF-BC.pdf}
        % \vspace{-12pt}
        \caption{Backdoor Criterion}
        \label{subfig:CNF-BC}
    \end{subfigure}
    
    \caption{Graphical models (top) encode desired (conditional) independencies.
    Structured generative networks (bottom) for learning BGMs are constructed according to the corresponding graphical models.
    Blue variables are sampled independently from Gaussian distributions while black variables are observed in the dataset.
    % The yellow CGM is not necessary in practice.}
    }
    \label{fig:CNF}
\end{figure}

In the \textbf{IV} (\S\ref{sub:IV}) and \textbf{BC} (\S\ref{sub:BC}) cases on the other hand, training is not as simple at the first glance.
We cannot sample $\hat{U}$ and $\boldsymbol{X}$ independently anymore, as they do not need to be independent.
Additionally, we need to satisfy the conditional independence constraints of each case.
% (first conditions in \Cref{thm:IV,thm:BC}).

To efficiently encode the conditional independence constraints, we use directed graphical models (DGM)~\cite{koller2009probabilistic} for building \emph{structured generative networks} which consist of CGMs as their building blocks, and inherit all conditional independencies encoded in the DGM.\footnote{Here, we treat DGMs as a pure statistical objects devoid of any causal semantics.}
\Cref{fig:CNF} demonstrates the DGMs used for satisfying the conditional independencies of IV and BC cases,
as well as
% \footnote{\Cref{app:CI} demonstrates several alternative DGMs that encode the same conditional independencies.}
% \Cref{fig:CNF} demonstrates 
structured generative models built according to these DGMs. Note that the shown DGMs and structured generative networks are not the only ones that satisfy the required conditional independence properties. In the BC case, there are several alternatives DGM that encode the same conditional independencies and each define a distinct structured generative network that could be used to learn $\hat{f}$ (see \Cref{app:CI}). Also note that the CGM used for representing $\hat{f}_{\theta}$ (green one) has requirements like monotonicity and differentiability, but the others do not have these restrictions.

\textbf{Training:}
We sample the root variables, $\boldsymbol{\epsilon}_{\boldsymbol{X}}, \epsilon_{\hat{U}}, \boldsymbol{I}$ in \Cref{subfig:CNF-IV}, and $\boldsymbol{\epsilon}_{\boldsymbol{X}}, \epsilon_{\hat{U}}, \boldsymbol{Z}$ in \Cref{subfig:CNF-BC}, independently. 
The epsilon variables (in blue) are sampled from independent Gaussian distributions, and the others from the dataset $\mathcal{D}$.
We train the whole structure end-to-end, with the goal of matching the distribution of $\mathcal{D}$.
This process is akin to a constrained search for $\hat{f}$ where the constraints are embedded in the search space by construction.
The objective function is determined by the choice of CGM.
We can even mix different types of CGMs, and combine different objective functions for their end-to-end optimization.

The end goal of training is to learn the green CGM.
As a result, any CGM whose training does not affect the green CGM can be removed from the network as a simplification.
The yellow CGM in \Cref{subfig:CNF-BC} is such an example, as it is surrounded by black variables that are sampled directly from $\mathcal{D}$, which prevent its gradients from passing through and influencing training of the other CGMs. 
%\todo{Is this too much explanation?}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% In \S\ref{sec:identifiability}, we demonstrated three different settings in which BGMs are identifiable (up to indeterminacies that are harmless for counterfactual estimation) from distributions.
% Therefore, fitting the data distribution is a proper objective for finding the underlying BGM in these cases.
% Each of these cases has an essential distributional constraint, denoted by the first constraint of the corresponding theorem.
% In this section, we present an efficient solution for modeling the joint data distribution subject to the distributional constraint.
% To this end, we make use of Conditional Generative Models (CGM) as building blocks for designing structured generative networks in the form of probabilistic graphical models in which the distributional constraint (independence or conditional independence) holds.
% This way, the distribution produced by the structured generative network is guaranteed to satisfy the distributional constraint, by design.

% There exist many types of CGMs based on different generative models, e.g., Normalizing Flows~\cite{papamakarios2021normalizing}, GANs, Denoising Probabilistic Diffusion Models~\cite{ho2020denoising} or score matching~\cite{song2019generative}, etc.
% Our models are mostly oblivious to the choice of CGM.
% We will highlight cases where this is not true.

% \subsection{The Markovian Case}
% The structured generative network for this case simply consists of a single CGM.
% Conditioned on the value of $\boldsymbol{X}$, this CGM is trained to map samples of $U \sim P_U$ where $P_U$ is an arbitrary distribution (typically Gaussian) to $P_{V|\boldsymbol{X}}$ samples.
% In training, we sample $U \sim P_U$ and $\boldsymbol{X}$ independently from each other which ensures the distributional constraint $(U \indep \boldsymbol{X})$ by construction.
% The last constraint of \Cref{thm:intervention} restricts us to strictly monotonic mappings for the CGM, e.g., strictly monotonic transforms used in Normalizing Flows.\footnote{NFs typically utilize transforms with efficient Jacobian to enable maximum likelihood training. 
% However, we do not have this requirement as we are oblivious to the training objective. 
% e.g., it is possible to use strictly monotonic mappings without tractable Jacobian to gain expressivity and faster convergence~\cite{si2021autoregressive}, and train them with adversarial loss (similar to GANs).}

% \subsection{Instrumental Variable (IV)}

% The structured generative network in this case is depicted in \Cref{subfig:CNF-IV}.
% It is designed to follow the directed graphical model in \Cref{subfig:PGM:CNF-IV} in which the two paths between $\boldsymbol{I}$ and $U$, $\boldsymbol{I} \rightarrow \boldsymbol{X} \leftarrow U$ and $\boldsymbol{I} \rightarrow \boldsymbol{X} \rightarrow V \leftarrow U$ are blocked by open v-structures (unconditioned $X$ and $\boldsymbol{V}$, respectively) which implies independence of $\boldsymbol{I}$ and $V$.\footnote{\label{foot1}Refer to \citet{pearl1988probabilistic,koller2009probabilistic} for details.}
% As a result, the distribution produced by the structured generative network is guaranteed to satisfy the distributional constraint $U \indep V$ (the first condition in \Cref{thm:IV}), by construction.
% In training, we sample $\boldsymbol{\epsilon}_{\boldsymbol{X}}, \epsilon_U$ from Gaussian distributions and $\boldsymbol{I}$ from the dataset, independently, and optimize the parameters of the CGMs to fit the distribution of $P_{\boldsymbol{X}, V|\boldsymbol{I}}$ in the dataset.
% In effect, this process efficiently searches the subspace of joint distributions over $U, V, \boldsymbol{I}, \boldsymbol{X}$ where $U \indep \boldsymbol{I}$, looking for the one that matches our dataset. 
% As proved by \Cref{thm:IV}, the solution for this constrained optimization is $g$-equivalent to the ground truth BGM.

% The only restriction we have for CGMs in this case is for the green one in \Cref{subfig:CNF-IV} that models the generation of $V$, which should be $C^2$-diffeomorphism according to the second constraint of \Cref{thm:IV}.
% Transforms used for designing NFs are diffeomorphisms and can be used for this CGM.
% However, they typically have efficient Jacobian, a requirement that we do not need in this case.
% Also, the transform we use in our experiments in \S\ref{x} is differentiable but not two times differentiable, so we believe that this assumption can be relaxed.


% \subsection{Backdoor Criterion (BC)}
% The distributional requirement we have in this case, i.e., $\boldsymbol{X} \indep U | \boldsymbol{Z}$ (first condition in \Cref{thm:BC}), is different from the previous two cases in that it is a conditional Independence property, as opposed to independence.
% However, our strategy for constraining the search space to networks that satisfy this constraint is the same as before.
% The structured generative network we build for this case (\Cref{subfig:CNF-BC}) resembles the structure of the directed graphical model shown in \Cref{subfig:PGM:CNF-BC}.
% As a result, it inherits all the conditional independence properties read off the graphical model using the $d$-separation test.\footref{foot1}
% There are two paths between $U$ and $\boldsymbol{X}$, $\boldsymbol{X} \leftarrow \boldsymbol{Z} \rightarrow U$ which is blocked when we condition on $\boldsymbol{Z}$, and $\boldsymbol{X} \rightarrow V \leftarrow U$ which is blocked due to the v-structure at $V$, thus $\boldsymbol{X} \indep U | \boldsymbol{Z}$.

% It is worth emphasizing that the directed graphical model used for constructing the structured generative network is purely a statistical object as opposed to a causal DAG, and its goal is solely to equip the structured generative network with the corresponding distributional constraint in each case.
% As a result, all directed graphical models in the Markovian equivalence class\footnote{Directed graphical models that encode the same conditional independencies.} of \Cref{subfig:PGM:CNF-BC} are valid and can be used for constructing alternative structured generative network, as we do in \Cref{app:alternative-BC}.

% The second condition in \Cref{thm:BC} requires the CGM used for $P_{V|\boldsymbol{X}}$ (green one in \Cref{subfig:CNF-BC}) to be a diffeomorphism, which makes NFs suitable candidates for this CGM. \todo{Combine this sentence for the three cases?}
% The third condition requires this transform (and its inverse) to be differentiable with respect to $\boldsymbol{X}$.
% However, this is not the case in our experiments in \S\ref{x}.
% As a result, we believe this technical condition can be relaxed.
% Also, recall that this generative modeling aims to find the BGM for $V$ by the green CGM, and other CGMs are merely used to enforce the distributional constraints.
% As a result, we could exclude the yellow CGM used for $P_{\boldsymbol{X}|Z}$ as its only connection with other CGMs is through $\boldsymbol{Z}$ and $\boldsymbol{X}$ through which no gradient flows because they are sampled from the dataset. 

==> sections/pre.tex <==
% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{booktabs} % for professional tables

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2023} with \usepackage[nohyperref]{icml2023} above.
\usepackage{hyperref}


% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}

% Use the following line for the initial blind version submitted for review:
% \usepackage{icml2023}

% If accepted, instead use the following line for the camera-ready submission:
\usepackage[accepted]{icml2023}

% For theorems and such
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}

% if you use cleveref..
\usepackage[capitalize,noabbrev]{cleveref}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

% Todonotes is useful during development; simply uncomment the next line
%    and comment out the line below the next line to turn off comments
%\usepackage[disable,textsize=tiny]{todonotes}
\usepackage[textsize=tiny]{todonotes}

\def\indep{\perp\!\!\!\perp}

% \newcommand{\edited}[1]{{\color{red}#1}}
\newcommand{\removed}[1]{{\color{purple}#1}}
\newcommand{\edited}[1]{#1}

\newcommand\footnoteref[1]{\protected@xdef\@thefnmark{\ref{#1}}\@footnotemark}

\newcommand{\ma}[1]{{\color{blue}M: #1}}
\newcommand{\arash}[1]{{\color{red}A: #1}}
\newcommand{\devavrat}[1]{{\color{green}D: #1}}
% \usepackage{romannum}

==> sections/problem.tex <==
\section{Problem Formulation}
\label{sec:problem}
We assume knowledge of the causal diagram $\mathcal{G}$ that might include unobserved confounders (no Markovianity assumption), and access to observational ($\mathcal{L}_1$)
% or interventional ($\mathcal{L}_2$) 
data \edited{distribution}.
We are interested in learning the data generation mechanisms $\mathcal{F}$, which can be further used for counterfactual $(\mathcal{L}_3)$ estimation.
As demonstrated by Pearl's Causal Hierarchy Theorem~\citep[Thm.~27]{bareinboim2022pearl}, cross-layer inference is not possible in general settings, and we need to make further assumptions.

\textbf{Bijective Generation Mechanism (BGM)}:
As mentioned in \S\ref{sec:prelim}, each endogenous variable $V_i$ is generated in the following way in the SCM framework:
\begin{equation}
\label{eqn:generation_mechanism}
    V_i \coloneqq f_i\Big(\text{Pa}(V_i), U_i\Big)
\end{equation}
We assume that the function $f_i$ is a bijective mapping from $U_i$ to $V_i$, for each realization of $\text{Pa}(V_i)$, hence the name \emph{Bijective Generation Mechanism (BGM)}.
In other words, no information is lost in transformation from exogenous to endogenous variables.
We refer to the inverse of the generation mechanism as $f_i^{-1}(\text{Pa}, \cdot)$, i.e.,
\begin{equation}
\label{eqn:reverse_generation_mechanism}
    U_i = f_i^{-1}\Big(\text{Pa}(V_i), V_i\Big).
\end{equation}
Note that the nonlinear ANM~\cite{peters2014causal}, LSNM~\cite{immer2022identifiability}, and PNL~\cite{zhang2009identifiability} models from prior work are all special cases of BGMs. Specifically, the nonlinear ANM model, 
\begin{equation}
    f_i\Big(\text{Pa}(V_i), U_i\Big) = g_i\Big(\text{Pa}(V_i)\Big) + U_i
\end{equation} LSNM~\cite{immer2022identifiability} model, 
\begin{equation}
    f_i\Big(\text{Pa}(V_i), U_i\Big) = l\Big(\text{Pa}(V_i)\Big) + s\Big(\text{Pa}(V_i)\Big)U_i
\end{equation}
with $s$ a strictly positive function on $\mathbb{R}$, 
%$l$ and $s$ being two-times differentiable functions defined on $\mathbb{R}$ and $s$ being strictly positive, 
and PNL causal models~\cite{zhang2009identifiability}, 
\begin{equation}
    f_i\Big(\text{Pa}(V_i), U_i\Big) = h_i\bigg(g_i\Big(\text{Pa}(V_i)\Big) + U_i\bigg)
\end{equation}
with $h_i$ an invertible function, are all bijective given $\text{Pa}(V_i)$.

%are all special cases of BGM, and widely used in the literature.

==> sections/related.tex <==
\section{Related Work}
\label{sec:related}

% \subsection{Interventional $(\mathcal{L}_2)$ Identification and Estimation}
\textbf{Interventional $(\mathcal{L}_2)$ Identification and Estimation}:
Assuming a coarse knowledge of the underlying system in the form of a causal DAG, identification of interventional queries has been extensively studied in the literature~\citep[Ch.~3]{pearl2009causality}, including \textit{do-calculus}~\cite{pearl1995causal} as a general solution. 
In cases where the full causal diagram is not accessible, another line of work focuses on its (partial) identification using observational data.
Although this sounds compelling and amenable to data-driven and ML research practices, it is known that the causal diagram can be identified from observational data only up to its Markovian equivalence class~\cite{spirtes2001causation}.
Investigating identifiability using only equivalence classes has thus received research attention~\cite{zhang2008completeness,perkovic2018complete,jaber2019causal}.
\citet{witti2021sbi} investigates a simulation-based notion of identifiability with probabilistic programs~\cite{goodman2008church}, using priors over parametric representations of SCMs.
Once identifability of the interventional query is established, various methods exist for estimation of the causal effect, including Propensity Score for the backdoor case~\cite{rubin1978bayesian,kennedy2019nonparametric}, and other statistical methods for more relaxed settings~\cite{fulcher2020robust,jung2020learning}.
In cases where the interventional query is non-identifiable, \emph{partial identification} methods estimate meaningful bounds~\cite{manski1990nonparametric,balke1997bounds,zhang2021bounding,li2022bounds}


\textbf{Counterfactual $(\mathcal{L}_3)$ Identification}:
Using the \emph{counterfactual graph}, \citet{shpitser2007counterfactuals} proposes an algorithm that determines identifiability of counterfactual queries from interventional data.
This was extended in \citet{correa2021nested} by providing sufficient and necessary graphical conditions for identification of (nested) counterfactuals from a collection of observational and interventional distributions, given the causal diagram.
In identifiable cases, these algorithms express the counterfactual query as a combination of observational and interventional quantities.
However, estimating this expression may not be tractable.
\citet{shah2022counterfactual} proves identifiability of counterfactuals for a specific causal diagram and provides an algorithm for their tractable estimation, assuming the joint distribution of exogenous and endogenous variables is an exponential family.
In contrast, we do not restrict the joint distribution of variables.

Similar to the interventional case, partial identification methods have been proposed for non-identifiable counterfactual queries~\cite{balke1994counterfactual,tian2000probabilities,finkelstein2020deriving,zhang2022partial,gresele22}.
Furthermore, identification of specific counterfactual queries has been studied in isolation, e.g., the \emph{effect of treatment on the treated}~\cite{shpitser2009effects}, \emph{path-specific effects}~\cite{shpitser2018identification,zhang2018fairness}, and \emph{probabilities of causation}~\cite{pearl1999probabilities}.


\textbf{Neural Methods for Causal Estimation\footnote{\Cref{app:related} provides a more detailed survey.}}:
There is a growing literature on applying neural methods for efficient estimation of causal queries.
An extensive line of work focuses on estimating interventional $(\mathcal{L}_2)$ queries including \citet{kocaoglu2018causalgan,xia2021causal,zevcevic2021relating}, to name a few.
However, we focus on estimating counterfactuals $(\mathcal{L}_3)$.

On the counterfactual side, a line of work uses ML techniques for estimation without any guarantees about the identifiability of the counterfactual query~\cite{pawlowski2020deep,khemakhem2021causal,sanchez2021vaca,sanchez2021diffusion,geffner2022deep}.
In contrast, we prove identifiability for several causal structures in \S\ref{sec:identifiability}. Furthermore, most existing techniques make restrictive assumptions about  the causal structure or generation mechanisms. For example, \citet{johansson2016learning,shalit2017estimating,yao2018representation,oberst2019counterfactual,lorberbom2021learning,xia2022neural} consider counterfactual estimation in domains with discrete (finite-valued) endogenous variables. Several others works assume a Markovian causal structure~\cite{pawlowski2020deep,khemakhem2021causal,sanchez2021vaca,geffner2022deep}, i.e., the absence of unobserved confounders (bidirected edges in the causal diagram).
\citet{hartford2017deep,khemakhem2021causal,geffner2022deep} restrict the class of generation mechanisms to Nonlinear Additive Noise Models (ANM)~\cite{hoyer2008nonlinear} or Location Scale Noise Models (LSNM)~\cite{strobl2022identifying}. The models we consider are more general than these prior papers. They support continuous endogenous variables, allow unobserved confounders, and bijective generation mechanisms that include nonlinear ANM, LSNM, and post-nonlinear causal model (PNL)~\cite{zhang2009identifiability} as special cases. 


\textbf{Disentanglement}:
Independent Component Analysis (ICA)~\cite{hyvarinen2000independent} concerns the problem of recovering statistically independent source signals $\boldsymbol{S} = (S_1, \ldots, S_n)$ from their observed mixtures $\boldsymbol{X} = (X_1, \ldots, X_n)$, where $\boldsymbol{X} = f(\boldsymbol{S})$, and the unknown $f$ (mixing function) is assumed to be invertible.
Unlike linear mixing functions that make this problem identifiable with certain conditions, it is known to be non-identifiable for non-linear mixing functions~\cite{hyvarinen1999nonlinear}.
Recently, \citet{hyvarinen2019nonlinear} proved identifiability in the presence of auxiliary variables, which make the sources conditionally independent.
This has been exploited for disentangling semantically meaningful features of high-dimensional data~\cite{locatello2019challenging,khemakhem2020variational}.

We took inspiration from the non-linear ICA framework, especially for our development in \S\ref{sub:BC}.
However, the problem we consider is fundamentally different: We are interested in disentangling the total contribution of the unknown sources of variation from known attributes, as opposed to disentangling the effect of individual unknown sources.
A recent work~\cite{shaham2022discovery} considers disentangling latent variables from observed attributes, and proves that the reconstructed sources $\hat{\boldsymbol{S}}$ have the same entropy as the true sources, in distribution.
However, we are interested in point-wise guarantees, i.e., $\hat{\boldsymbol{s}} = g(\boldsymbol{s})$ for some invertible function $g(\cdot)$, which are stronger than the distributional properties like $\mathcal{H}(\hat{\boldsymbol{S}}) = \mathcal{H}(\boldsymbol{S})$.
